Parameter learning and fractional differential operators: application in image regularization and decomposition

In this paper, we focus on learning optimal parameters for PDE-based image regularization and decomposition. First we learn the regularization parameter and the differential operator for gray-scale image denoising using the fractional Laplacian in combination with a bilevel optimization problem. In our setting the fractional Laplacian allows the use of Fourier transform, which enables the optimization of the denoising operator. We prove stable and explainable results as an advantage in comparison to other machine learning approaches. The numerical experiments correlate with our theoretical model setting and show a reduction of computing time in contrast to the ROF model. Second we introduce a new image decomposition model with the fractional Laplacian and the Riesz potential. We provide an explicit formula for the unique solution and the numerical experiments illustrate the efficiency.

==> paper_bib.tex <==
@article{AntBar17,
  author = {Antil, Harbir and Bartels, S\"{o}ren},
  title = {Spectral approximation of fractional {PDE}s in image
              processing and phase field modeling},
  journal = {Comput. Methods Appl. Math.},
  fjournal = {Computational Methods in Applied Mathematics},
  volume = {17},
  year = {2017},
  number = {4},
  pages = {661--678},
  issn = {1609-4840},
  mrclass = {65N35 (26A33 35R11 35S05 49K20 49M05 65N12)},
  mrnumber = {3709055},
  doi = {10.1515/cmam-2017-0039},
  url = {https://doi.org/10.1515/cmam-2017-0039},
  pdf = {articles-pre/AntBar17-pre.pdf}
}

@article {AntOtaSal18,
	AUTHOR = {Antil, Harbir and Ot\'{a}rola, Enrique and Salgado, Abner J.},
	TITLE = {Optimization with respect to order in a fractional diffusion
	model: analysis, approximation and algorithmic aspects},
	JOURNAL = {J. Sci. Comput.},
	FJOURNAL = {Journal of Scientific Computing},
	VOLUME = {77},
	YEAR = {2018},
	NUMBER = {1},
	PAGES = {204--224},
	ISSN = {0885-7474},
	MRCLASS = {65N21 (26A33 35J70 35R11 49J20 49K21 49M25)},
	MRNUMBER = {3850351},
	MRREVIEWER = {An\'{\i}bal Coronel},
	DOI = {10.1007/s10915-018-0703-0},
	URL = {https://doi.org/10.1007/s10915-018-0703-0},
}

@book {BoyFab13,
	AUTHOR = {Boyer, Franck and Fabrie, Pierre},
	TITLE = {Mathematical tools for the study of the incompressible
	{N}avier-{S}tokes equations and related models},
	SERIES = {Applied Mathematical Sciences},
	VOLUME = {183},
	PUBLISHER = {Springer, New York},
	YEAR = {2013},
	PAGES = {xiv+525},
	ISBN = {978-1-4614-5974-3; 978-1-4614-5975-0},
	MRCLASS = {76-02 (35Q30 35Q35 76D05)},
	MRNUMBER = {2986590},
	MRREVIEWER = {Isabelle Gruais},
	DOI = {10.1007/978-1-4614-5975-0},
	URL = {https://doi.org/10.1007/978-1-4614-5975-0},
}
